Convergence of a Human-in-the-Loop Policy-Gradient Algorithm With Eligibility Trace Under Reward, Policy, and Advantage Feedback

Fluid human-agent communication is essential for the future of human-in-the-loop reinforcement learning. An agent must respond appropriately to feedback from its human trainer even before they have significant experience working together. Therefore, it is important that learning agents respond well to various feedback schemes human trainers are likely to provide. This work analyzes the COnvergent Actor-Critic by Humans (COACH) algorithm under three different types of feedback-policy feedback, reward feedback, and advantage feedback. For these three feedback types, we find that COACH can behave sub-optimally. We propose a variant of COACH, episodic COACH (E-COACH), which we prove converges for all three types. We compare our COACH variant with two other reinforcement-learning algorithms: Q-learning and TAMER.

==> TODO2.tex <==
TODO:

- Fix graphs.  Make TAMER





- Konda paper

TO DO Ishaan:
Add $\pi$ in the expectation everywhere


DONE Ishaan Confirm:

Update comparison section on q-learning for indicator in finite horizon

- Explain pseudocode.  Talk about versions of TAMER and the one we're using


DONE David Confirm:
- Add more clarification on differences between COACH and E-COACH.

- Show why COACH does not converge.  Or clarify things

==> TODO3.tex <==
Theorem 2 seems shakey. For example, Assumption 1 seems weird when there are multiple optimal policies. And, why limit to finite horizons?
-Notes:  Requires big restructure of theorem 2.  We should spend time thinking about this.  And maybe ask Kavosh for advice.
What we did:  Added more to the theorem for the infinite horizon case


“We can leverage Theorem 2 to show that the algorithm converges under policy feedback.“: Are the assumptions needed or are they satisfied by the way Theorem 3 is constructed?
-Notes:  Confused by this.  Assumptions should be the same for both.  But assumptions should only hold in section 4.
What we did:  Changed the assumptions being referred to here.  May still need to add clarification.


“The algorithm will converge,“: To what? I think saying what it   converges to will make the rest of the (short) section clearer. Similarly, Section 6.2 is unclear.
-Notes:  Common theme.  Need to fix in multiple places.  Converges to what?
-Gradient does not necessarily converge.  

What can we say about TAMER and Q-learning theoretically? I believe that interesting results about these algorithms would go a long way to making the paper stand out.
-Notes:  Something to look into.  Will Q-Learning converge with the policy as a parameter as well?

Empirically, it looks like Q-learning is the way to go. What’s the   deal?
-Notes:  Yup.  Q-Learning is great.

We should ask James what he thinks about the analysis. It’s possible we’re misunderstanding COACH.
-Notes:  I think Michael is referring to section 6 here.  Could ask James.
What we did: Emailed.  Waiting for response

Regarding Figure 1, I’m concerned about the use of average reward. In particular, we kind of made a fuss about how important it is the get discounting correct. Could we compute the regret of the learned policy instead? (All three plots should be on the same scale, too.)
-Notes:  Check if reward is discounted.  Change to ``Average Value.''  Look into regret (might be difference between given policy and optimal policy?).
What we did:  There's now an option to have experiments for discounted award instead of non-discounted

We should do some kind of empirical comparison between COACH and E-COACH.
-Notes:  They're made for different things.  But could be good to show that E-COACH succeeds on tasks that COACH does not.  Maybe just run COACH as E-COACH without discounting.

Any chance we could include another environment, perhaps a deep RL experiment?
-Notes:  We could look into this.  We should also look into an RL package that isn't simple\_rl.  We did try it in mountain car, we found that E-COACH needs immediate reward to learn.  It does a poor job exploring.

Work through what E-Coach’s update is in the tabular setting. (It works, right?)
-Notes:  This is what we were doing in our experiments.  We aren't sure it works in the non-tabular setting (?).

Questions for James:
-What does he think of our analysis of COACH in section 6.
-What does he think of our changes to COACH to create E-COACH.

Questions for Kavosh:
-What does he think about section 4 and Michael's comments on that section.  Could we make it cleaner?



Notes:
Consider removing the term convergence before each section. On the other hand, the paper is called "Convergence of a Human-in ..." so we would like to talk about convergence at some point.

==> content/experiments.tex <==
\section{Experiments}
\label{experimentsSection}
We used the simple\_rl framework (zzz ref) to test the performance of E-COACH in different grid worlds under different feedback schemes. 
% We examined COACH agents with different feedback schemes. 
% The first one received the MDP's reward function $R(s,a)$ as feedback while the second one received $I(s,a)$ (as described in Section~\ref{indicatorSection}). 
To generate an optimal policy for action feedback, 
% $I(s,a)$
we ran value iteration (VI) on the MDP for a large number of iterations (zzz be more specific) before the start of learning.
% hand to compute $\pi^{*}$. We compared the discounted 
% average (zzz averaged over what?)  (Averaged over multiple instances.  Not worth mentioning.)
reward obtained by {Q}-learning (zzz why Q learning? Why not show pi start?) and a random agent to that of the three E-COACH agents. 
% (why two and not all three?)

% TODO WORKING ON THIS
\begin{figure}
    \centering
    \begin{subfigure}
        \centering
        \includegraphics[width=0.4\textwidth]{content/graphics/average_reward3.pdf}
        \caption{E-COACH on $3 \times 3$ Gridworld with Lava}
        \label{3by3}
    \end{subfigure}
    % \hfill %
    \begin{subfigure}
        \centering
        \includegraphics[width=0.4\textwidth]{content/graphics/average_reward10.pdf}
        \caption{E-COACH on $10 \times 10$ Gridworld with Lava}
        \label{10by10}
    \end{subfigure}
    % \caption{COACH on Gridworld with Lava}
    % \label{gridworldExperiments}
\end{figure}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\columnwidth]{content/graphics/average_reward3.pdf}
%     \caption{$3 \times 3$}
%     \label{3by3}
% \end{figure}

% \begin{figure}[h]
% \centering
%     \begin{subfigure}[h]{0.4\columnwidth}
%         \includegraphics[width=\linewidth]{content/graphics/average_reward3.pdf}
%         \caption{Caption}
%         \label{fig:my_label}
%     \end{subfigure}
%     \begin{subfigure}[h]{0.4\columnwidth}
%         \includegraphics[width=\linewidth]{content/graphics/average_reward10.pdf}
%         \caption{Caption}
%     \end{subfigure}
%     % \subfigure{\includegraphics[0.45\textwidth]{content/graphics/average_reward3.pdf}}
%     % \hspace{0.05\textwidth}
%     % \subfigure{\includegraphics[0.45\textwidth]{content/graphics/average_reward10.pdf}}
% \end{figure}

% \begin{figure}[h]{width=\linewidth}
%   \begin{subfigure}[b]{0.4\columnwidth}
%     \includegraphics[width=\linewidth]{content/graphics/average_reward3.pdf}
%     \caption{Picture 1}
%     \label{fig:1}
%   \end{subfigure}
%   \hfill %%
%   \begin{subfigure}[b]{0.4\columnwidth}
%     \includegraphics[width=\linewidth]{content/graphics/average_reward10.pdf}
%     \caption{Picture 2}
%     \label{fig:2}
%   \end{subfigure}
% \end{figure}


As seen in the results in Figure~\ref{3by3} and \ref{10by10}, the two E-COACH agents perform nearly optimally. In the $3\times 3$ gridworld, the two E-COACH agents converge at a slower rate than {Q}-learning but eventually catch up with it. In the $10\times 10$ gridworld, the two E-COACH agents consistently outperform {Q}-learning. It is interesting to note that the graphs for the two E-COACH agents are very similar even though they receive very different feedback. (zzz why the difference relative to {Q}-learning? Why did 3x3 run longer than the more complex 10x10?)

==> content/indicator_function/old/indicator_function_main_old.tex <==
\section{Convergence Under Policy Feedback}
% NOTE MIGHT WANT https://people.eecs.berkeley.edu/~pabbeel/cs287-fa09/readings/NgHaradaRussell-shaping-ICML1999.pdf TO SHOW INVARIANCE OF REWARD FUNCTION.  WE CAN CHOOSE V_{MIN} >= 0

To argue that E-COACH converges under policy feedback, we first consider a more general form of feedback and then show policy feedback is a special case.

\subsection{Convergence of a More General Type of Feedback}
\label{generalization}

Let us start by considering two similar MDPs $M_1 = \langle S, A, R, T, \gamma\rangle$ and $M_2 = \langle S, A, f, T, \gamma\rangle$, where we assume $\lambda \in [0, 1)$.  Note the differing reward functions $R$ and $f$ in the two MDPs.

We will denote the value functions for $M_1$ and $M_2$ as $V_1$ and $V_2$, respectively.  We will say that the starting state for both of our MDPs is $s_0$. Define $V_1^{\min} = \min_{\pi \in \Pi} V_1^\pi (s_0)$, $V_1^{*} = \max_{\pi \in \Pi} V_1^\pi(s_0)$.

The following theorem will have the following assumption:

% \textbf{Assumption:}
\begin{enumerate}
    \item E-COACH (see algorithm \ref{coachAlgorithm}) will give us a policy $\pi_2(s, a)$ such that $\fa s, \sum_a | \pi_2(s, a) - \pi_2^*(s, a)| < \delta$ for some optimal policy $\pi_2^*$ on the domain $M_2$.  Note $\pi_2^*$ may not be the only optimal policy; instead, it is a single optimal policy.  This assumption is substantiated by the proof in Section~\ref{oneStepRewardSection}, which ensures convergence to a local maximum. \label{kavoshAssumption}
    \item We also assume that $\gamma \neq 1$ for the case where the MDP has an infinite horizon, which will we will justify later on. \label{lambdaNotOneAssumption}
\end{enumerate}
\thmNum{genThmNum}
\textbf{Theorem~\ref{genThmNum}:} If all optimal policies for $M_2$ are also optimal for $M_1$ (optimal policies of $M_2$ are a subset of those for $M_1$), then running E-COACH on $M_2$ will result in a policy that is close to an optimal policy on $M_2$, which will also be close to an optimal policy for $M_1$.  
Then in the finite horizon case with horizon limit $L$,
\begin{align*}
    (1 - \delta)^L V_1^{*} + (1 - (1 - \delta)^L)V_1^{\min} \leq V_1^{\pi_2} \leq V_1^{*}.
\end{align*}
And in the infinite horizon case,
\begin{align*}
    \lim_{\delta \rightarrow 0} V_1^* - V_1^{\pi_2} = 0
\end{align*}

\textbf{Proof:} 
Will will split this proof into cases, starting with the finite horizon case.  For this case, we will assume a termination time of $L$ on MDP $M_1$.
\subsubsection*{Proof of Theorem \ref{genThmNum} in Finite Horizon Case}
We have to show that running E-COACH in $M_2$ will yield a policy that is not too far off from an optimal policy for $M_1$.  We would like to run E-COACH on $M_2$, using the alternate form of feedback as the reward function, and for any good policy we get from E-COACH on $M_2$, we would like for that policy to also be good on $M_1$, the original MDP we are trying to solve.  

We're interested in the value function over $M_1$, but using the policy given from E-COACH (under one-step-reward) on $M_2$, and we will call this policy $\pi_2$.  We would like the value function under $\pi_2$ to be close to optimal, $V_1^{*}$.  Since $\pi_2$ cannot be better than optimal, we have that $V_1^{\pi_2} \leq V_1^{*}$.  This relation provides our upper bound. 
% Now, let us move to the lower bound.

The probability that the learner makes the exact optimal decision every time is at least $(1 - \delta)^L$, where $L$ is the termination time on $M_1$.
Then, the probability we take a wrong action at some point would be $(1 - (1 - \delta)^L)$, and we can lower bound the punishment from making this wrong move by assuming $V_1^{\min}$.
Now, we have a lower bound:
\begin{align*}
    (1 - \delta)^L V_1^{*}(s_0) + (1 - (1 - \delta)^L) V_1^{\min} \leq V_1^{\pi_2}(s_0)
\end{align*}

Combining the upper and lower bound, we have that
\begin{align*}
    (1 - \delta)^L V_1^{*}(s_0) + (1 - (1 - \delta)^L) V_1^{\min} \leq V_1^{\pi_2} \leq V_1^{*}(s_0)
\end{align*}
If successful, E-COACH (under one-step-reward) will return to us a policy that is very nearly optimal.  In other words, $\sum_a|\pi_2(s, a) - \pi_2^*(s, a)|$ is close to zero, meaning $\delta \approx 0$, tightening the lower bound because $(1 - \delta)^L \approx 1$ and $(1 - (1 - \delta)^L) \approx 0$.\footnote{Note, however, that any error is compounded $L$ times.}  

Clearly, the distance our policy is off from $V_1^{*}$ would be:
\begin{align*}
    V_1^{*} - V_1^{\pi_2} \leq (1 - (1 - \delta)^L) (V_1^{*} - V_1^{\min})
\end{align*}
We can conclude that the policy given by running E-COACH on $M_2$ yields a policy that works well on $M_1$ in the finite horizon case.  Now let's move on to the infinite horizon case.

\subsubsection{Proof of Theorem \ref{genThmNum} in Infinite Horizon Case}
Let $\pi_2$ be the policy obtained by running E-COACH on $M_2$.  By the assumption shown above, we know that there exists a policy $\pi_2^*$ such that $\sum_a | \pi_2^*(s, a) - \pi_2(s, a)| < \delta$.  By construction of the theorem, $\pi_2^*$ must also be an optimal policy in $M_1$.  

Let $s = \argmax_{s' \in S} (V_1(s') - V_1^{\pi_2}(s'))$.  Define the set $A'_s$ to contain all actions, $a_0$, such that $\pi_2^*(s, a_0) > 0$.  Then by definition, for any $a_0 \in A_s$ we have that $Q^*_1(s, a_0) = \max_{a'} Q^*(s, a')$.  Let's also select $a = \argmin_{a' \in A'_s}Q^{\pi_2}(s, a')$.  We will let $W = \max_{s' \in S}(V_1^*(s') - V_1^{\pi_2}(s'))$ and notice that $W \geq 0$.

From the assumption listed above, we can safely say the following with similar reasoning to that in the finite horizon section:
\begin{align*}
    V_1^{\pi_2}(s) \geq (1 - \delta) Q_1^{\pi_2}(s, a) + \delta V_1^{\min}
\end{align*}
If successful, E-COACH will return to us a policy that is near optimal, otherwise we can assume worst-case scenario, which achieves $V_1^{\min}$.

From the previous equation, we can say that $V_1^{\pi_2}(s) \geq (1 - \delta) (R(s, a) + \gamma \sum_{s_2 \in S} T(s_1 \given a, s) V_1^{\pi_2}(s_2)) + \delta V_1^{\min}$.

Notice the following:
\begin{align*}
    V_1^*(s) = R(s, a) + \gamma \sum_{s_2 \in S} T(s_2 \given a, s) V_1^* (s_2)
\end{align*}

Now let's reintroduce $W$, using the above terms.

\begin{align*}
    W =& V_1^*(s) - V_1^{\pi_2}(s) \\
    \leq& \delta(V_1^*(s) - V_1^{\min}) + \\
    &(1 - \delta) (\gamma \sum_{s_2 \in S} T(s_2 \given a, s) (V_1^*(s_2) - V_1^{\pi_2}(s_2)))
\end{align*}
Note that $W \geq V_1^*(s_2) - V_1^{\pi_2}(s_2)$.  From this we can say that\ldots
\begin{align*}
    W& \leq \delta(V_1^*(s) - V_1^{\min}) + (1 - \delta) \gamma W
\end{align*}
Which implies that\ldots
\begin{align*}
    (1 - (1 - \delta) \gamma) W& \leq \delta (V_1^*(s) - V_1^{\min})
\end{align*}
Which further implies that\ldots
\begin{align*}
    W \leq \frac{\delta}{(1 - (1 - \delta) \gamma)} (V_1^* (s) - V_1^{\min})
\end{align*}
Now let's consider this upper bound in the limit as $\delta \rightarrow 0$.  Recall that $0 \leq \gamma < 1$.  We have that\ldots
\begin{align*}
    &\lim_{\delta \rightarrow 0} \frac{\delta}{(1 - (1 - \delta) \gamma)} (V_1^* (s) - V_1^{\min}) = \\
    &(V_1^* (s) - V_1^{\min}) \cdot \lim_{\delta \rightarrow 0} \delta \cdot \lim_{\delta \rightarrow 0} \frac{1}{1 - (1 - \delta)\gamma} = \\
    &(V_1^* (s) - V_1^{\min}) \cdot 0 \cdot \frac{1}{1 - \gamma} = 0
\end{align*}
An MDP with $\gamma = 1$ would either accumulate infinite award forever, in which case the MDP is trivial and not useful for our practical purposes, or the MDP can easily be mapped to one with a finite horizon.

We have shown that $\lim_{\delta \rightarrow 0} W = 0$.  This means that the policy we get from running E-COACH on $M_2$ will work well on $M_1$ as well.  In the limit as $\lambda \rightarrow 0$, this policy will yield reward equivalent to that of an optimal policy.  \endproof

Note that our theorem says something different than the Simulation Lemma \cite{sim-lemma} as we make no assumptions about how close the reward functions of $M_1$ and $M_2$ are. Instead our theorem requires optimal policies in $M_2$ be optimal in $M_1$ and bounds the return of a policy learnt by E-COACH in $M_2$.  

\input{content/indicator_function/indicator_function_convergence.tex}

==> content/indicator_function/old/indicator_function_main_older.tex <==
\section{Convergence Under Policy Feedback}
% NOTE MIGHT WANT https://people.eecs.berkeley.edu/~pabbeel/cs287-fa09/readings/NgHaradaRussell-shaping-ICML1999.pdf TO SHOW INVARIANCE OF REWARD FUNCTION.  WE CAN CHOOSE V_{MIN} >= 0

To argue that E-COACH converges under policy feedback, we first consider a more general form of feedback and then show policy feedback is a special case.

\subsection{Convergence of a More General Type of Feedback}
\label{generalization}

Let us start by considering two similar MDPs $M_1 = \langle S, A, R, T, \gamma\rangle$ and $M_2 = \langle S, A, f, T, \gamma\rangle$.  Note the differing reward functions $R$ and $f$ in the two MDPs.

We will denote the value functions for $M_1$ and $M_2$ as $V_1$ and $V_2$, respectively.  We will say that the starting state for both of our MDPs is $s_0$. Define $V_1^{\min} = \min_{\pi \in \Pi} V_1^\pi (s_0)$, $V_1^{*} = \max_{\pi \in \Pi} V_1^\pi(s_0)$, and $L$ to be the termination time of $M_1$.

\textbf{Assumptions:}
\begin{enumerate}
    % \item The REINFORCE (Algorithm~\ref{reinforceAlgorithm}) will give us a policy $\pi_2(s, a)$ such that $\fa s, \sum_a | \pi_2(s, a) - \pi_2^*(s, a) | < \delta$ for some optimal policy $\pi_2^*$ on the domain $M_2$.  Note $\pi_2^*$ may definitely not be the only optimal policy; instead, it's a single optimal policy.  \label{kavoshAssumption} 
    % (zzz What's the status of this assumption? is it known to be false? Sorry, I'll be more direct. This assumption has got to be false in general. After all, two very different policies can both be optimal. So, there's no way in general that policy gradient or any other RL algorithm would return similar policies on two MDPs. So, when, if ever, would this assumption be meaningful? ALSO, I don't think we've defined what we mean by ``the policy gradient algorithm''. so a reference and explanation are needed.)  ADJUSTED
    \item E-COACH (see algorithm \ref{coachAlgorithm}) will give us a policy $\pi_2(s, a)$ such that $\fa s, \sum_a | \pi_2(s, a) - \pi_2^*(s, a)| < \delta$ for some optimal policy $\pi_2^*$ on the domain $M_2$.  Note $\pi_2^*$ may not be the only optimal policy; instead, it is a single optimal policy.  This assumption is substantiated by the proof in Section~\ref{oneStepRewardSection}, which ensures convergence to a local maximum. \label{kavoshAssumption}
    % \item The domains for $M_1$ and $M_2$ are communicating~\cite{puterman}, meaning the agent can reach any state from any other state with non-zero probability. \label{putermanAssumption}
    
    % does not have any states from which the  cannot return.  Like a ``black hole'' state.  In other words, you can get to any state from any other state.
    \item The MDPs $M_1$ and $M_2$ are MDPs with finite horizons.
\end{enumerate}
\thmNum{genThmNum}
\textbf{Theorem~\ref{genThmNum}:} If all optimal policies for $M_2$ are also optimal for $M_1$ (optimal policies of $M_2$ are a subset of those for $M_1$), then running E-COACH on $M_2$ will result in a policy that is close to an optimal policy on $M_2$, which will also be close to an optimal policy for $M_1$.  
Then,
\begin{align*}
    (1 - \delta)^L V_1^{*} + (1 - (1 - \delta)^L)V_1^{\min} \leq V_1^{\pi_2} \leq V_1^{*}.
\end{align*}

\textbf{Proof:} 
We have to show that running E-COACH in $M_2$ will yield a policy that is not too far off from an optimal policy for $M_1$.  We would like to run E-COACH on $M_2$, using the alternate form of feedback as the reward function, and for any good policy we get from E-COACH on $M_2$, we would like for that policy to also be good on $M_1$, the original MDP we are trying to solve.  

We're interested in the value function over $M_1$, but using the policy given from E-COACH (under one-step-reward) on $M_2$, and we will call this policy $\pi_2$.  We would like the value function under $\pi_2$ to be close to optimal, $V_1^{*}$.  Since $\pi_2$ cannot be better than optimal, we have that $V_1^{\pi_2} \leq V_1^{*}$.  This relation provides our upper bound.  
% Now, let us move to the lower bound.

The probability that the learner makes the exact optimal decision every time is at least $(1 - \delta)^L$, where $L$ is the termination time on $M_1$.
Then, the probability we take a wrong action at some point would be $(1 - (1 - \delta)^L)$, and we can lower bound the punishment from making this wrong move by assuming $V_1^{\min}$.
Now, we have a lower bound:
\begin{align*}
    (1 - \delta)^L V_1^{*}(s_0) + (1 - (1 - \delta)^L) V_1^{\min} \leq V_1^{\pi_2}(s_0)
\end{align*}

Combining the upper and lower bound, we have that
\begin{align*}
    (1 - \delta)^L V_1^{*}(s_0) + (1 - (1 - \delta)^L) V_1^{\min} \leq V_1^{\pi_2} \leq V_1^{*}(s_0)
\end{align*}
If successful, E-COACH (under one-step-reward) will return to us a policy that is very nearly optimal.  In other words, $\sum_a|\pi_2(s, a) - \pi_2^*(s, a)|$ is close to zero, meaning $\delta \approx 0$, tightening the lower bound because $(1 - \delta)^L \approx 1$ and $(1 - (1 - \delta)^L) \approx 0$.\footnote{Note, however, that any error is compounded $L$ times.}  

Clearly, the distance our policy is off from $V_1^{*}$ would be:
\begin{align*}
    V_1^{*} - V_1^{\pi_2} \leq (1 - (1 - \delta)^L) (V_1^{*} - V_1^{\min})
\end{align*}
We can conclude that the policy given by running E-COACH on $M_2$ yields a policy that works well on $M_1$. \endproof

Note that our theorem says something different than the Simulation Lemma \cite{sim-lemma} as we make no assumptions about how close the reward functions of $M_1$ and $M_2$ are. Instead our theorem requires optimal policies in $M_2$ be optimal in $M_1$ and bounds the return of a policy learnt by E-COACH in $M_2$.  

\input{content/indicator_function/indicator_function_convergence.tex}

==> content/old_conclusion.tex <==
% \section{Conclusion}
% \begin{figure}[h]
%     \centering
%     \begin{center}
%         \begin{tabular}{l | c c c}
%              Algorithm & $A(s, a)$ & $R(s, a)$ & $I(s, a)$ 
%               \\ \hline  \\
%              {Q}-learning & ? & \checkmark & ? \\
%              TAMER & ? & ? & ? \\
%              COACH & \checkmark & \checkmark & \checkmark
             
%         \end{tabular}
%     \end{center}
%     \caption{Convergence Under Various Algorithms}
%     \label{convergenceTable}
    
% \end{figure}

% We showed formally and empirically that COACH converges to optimal behavior under three important types of feedback.
% %This fact means a COACH agent is capable learning from several kinds of feedback that a human trainer might give.
% % We have shown that COACH will converge under any type of feedback, as long as the optimal policy under that feedback is the same as the optimal policy with the reward function as feedback. (zzz I don't understand this claim.)

% (zzz wouldn't {Q}-learning also do ok with I for the reasons you wrote up? I think if we define TAMER, it should be immediate that it can also learn from I. Maybe you need to be clear, though, that the I case depends on infinite horizon problems. Is that right? Or is it also ok with a pre-determined T? Could we run all three algorithms on all 3 feedbacks, even if we don't have formal results for all of them?)

% zzz references: use conference version of COACH paper. Spell out "NIPS". Provide venue for Thomas and Brunskill.


